OLViT: Multi-Modal State Tracking via Attention-Based Embeddings for Video-Grounded Dialog

We present the Object Language Video Transformer (OLViT) - a novel model for video dialog operating over a multi-modal attention-based dialog state tracker. Existing video dialog models struggle with questions requiring both spatial and temporal localization within videos, long-term temporal reasoning, and accurate object tracking across multiple dialog turns. OLViT addresses these challenges by maintaining a global dialog state based on the output of an Object State Tracker (OST) and a Language State Tracker (LST): while the OST attends to the most important objects within the video, the LST keeps track of the most important linguistic co-references to previous dialog turns. In stark contrast to previous works, our approach is generic by nature and is therefore capable of learning continuous multi-modal dialog state representations of the most relevant objects and rounds. As a result, they can be seamlessly integrated into Large Language Models (LLMs) and offer high flexibility in dealing with different datasets and tasks. Evaluations on the challenging DVD (response classification) and SIMMC 2.1 (response generation) datasets show that OLViT achieves new state-of-the-art performance across both datasets.

==> src/abstract.tex <==
\begin{abstract}
    We present the $\mathbb{O}$bject $\mathbb{L}$anguage $\mathbb{V}$ideo $\mathbb{T}$ransformer (\olvit) -- a novel model for video dialog operating over a multi-modal attention-based dialog state tracker.
    Existing video dialog models struggle with questions requiring both spatial and temporal localisation within videos, long-term temporal reasoning, and accurate object tracking across multiple dialog turns.
    \olvit\, alleviates these challenges by maintaining a global dialog state based on the output of an Object State Tracker (OST) and a Language State Tracker (LST):
    while the OST attends to the most important objects within the video, the LST keeps track of the most important linguistic co-references to previous dialog turns.
    Experimental results show that \olvit\, achieves a new state-of-the-art performance of $\mathbf{54.84\%}$ on the challenging DVD dataset corresponding to an improvement of $\mathbf{3.75\%}$ absolute points over the state of the art.
    Moreover, it outperforms strong baselines on the generative task of SIMMC 2.0 by reaching BLEU-4 scores of $\mathbf{0.283}$ and $\mathbf{0.252}$ on the \textit{test-dev} and \textit{test-std} splits corresponding to relative improvements of $\mathbf{30.4\%}$ and $\mathbf{20.0\%}$, respectively.
\end{abstract}

==> src/limitations.tex <==
\section{Limitations}
Although we achieved promising results on two challenging datasets, our work still suffers from two clear limitations: 
First, our model has been only applied on synthetic datasets with varying levels of realism.
This limitation is due to the lack of real-world and bias-free video dialog datasets that specifically test for higher-order reasoning.
Second, as depicted in \textcolor{myblue}{Table 1}, our model only managed to marginally outperform the current state of the art on the two question categories ``\textit{compare action seq}'' and ``\textit{compare action freq}''.
This might suggest that the reasoning over the whole video segment is still a daunting task for our model.
We are currently researching how we can overcome these limitations and improve our model's reasoning capabilities even further.

\section{Potential Risks}
Because our work relies on DistillRoBERTa, it suffers from the same potential risks as other established pre-trained language models \cite{zhu2019deep,9152761,risk}.
Moreover, since we showcased its efficacy on the SIMMC 2.0 task which emulates a shopping scenario, it might be maliciously used against customers' free will to persuade them to buy unnecessary or fake goods.
